Code Ownership: The Principles, Differences, and Their Associations with Software Quality

Code ownership -- an approximation of the degree of ownership of a software component -- is one of the important software measures used in quality improvement plans. However, prior studies proposed different variants of code ownership approximations. Yet, little is known about the difference in code ownership approximations and their association with software quality. In this paper, we investigate the differences in the commonly used ownership approximations (i.e., commit-based and line-based) in terms of the set of developers, the approximated code ownership values, and the expertise level. Then, we analyze the association of each code ownership approximation with the defect-proneness. Through an empirical study of 25 releases that span real-world open-source software systems, we find that commit-based and line-based ownership approximations produce different sets of developers, different code ownership values, and different sets of major developers. In addition, we find that the commit-based approximation has a stronger association with software quality than the line-based approximation. Based on our analysis, we recommend line-based code ownership be used for accountability purposes (e.g., authorship attribution, intellectual property), while commit-based code ownership should be used for rapid bug-fixing and charting quality improvement plans.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex

BIBTEX_FILES = \
	mybibfile.bib 

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	# open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> sections/confounding_factor.tex <==

% , which are listed in Tables \ref{Table:CodeMetrics} and \ref{Table:ProcessMetrics}.
% \textbf{Ownership metrics} describe the relationship between the ownership of modules and software quality~\cite{rahman2011ownership,thongtanunam2016revisiting,Bird2011a}.
% Following the traditional code ownership heuristics of Bird~\ea~\cite{Bird2011a}, for each module, we first measure the ownership of each developer using the proportion of the code changes made by the developer on the total code changes.
% We consider two granularities of code changes, i.e., lines of code level (LINE), and commit level (COMMIT).
% Second, we classify contributors into two levels of ownership of a module, as recommended by Bird~\ea~\cite{Bird2011a}.
% contributors with low code ownership (i.e., less than 5\% code contribution on a module) are considered as minor authors.
% On the other hand, contributors with high code ownership (i.e., more than 5\% code contribution on a module) are considered as major authors.
% In our study, we collect the number of the owner (i.e., the developer with the highest code contribution on a module), minor authors, and major authors with respective to the two granularities of code changes.



% \textbf{}{Product metrics} measure the characteristics of the source code of the released version. 
% The product metrics measure code characteristics in three dimensions: (1) complexity, e.g., McCabe Cyclomatic, (2) volume, e.g., lines of code, and (3) object-oriented design, e.g., coupling between object classes.
% The product metrics are computed using the \texttt{Understand} tool.
% % \footnote{\url{https://www.scitools.com/}}
% Due to the space limitation, we refer the detailed explanation of each product metric to the SciTools website.
% Since some product metrics are computed at the method level, we select three aggregation schemes (i.e., min, max, and average) to aggregate these metrics to the file level.
% Table~\ref{Table:CodeMetrics} provides a summary of the studied code metrics.
 % method-level software metrics to the file-level. 
% Our studied systems are based on Java where each file contains one class.
% Since some metrics are computed at the method level (e.g., cyclomatic), we aggregate such metrics to the file level using min, max, and mean.

% \textbf{Process metrics} measure the development activity during the development cycle of a release.
% For each file, the process metrics measure the number of commits (COMM), the number of lines added (ADDED\_LINES), the number of lines deleted (DEL\_LINES), the number of active contributors (ADEV), and the number of distinct contributors (DDEV).
% Similar to Rahman~\ea~\cite{rahman2013and}, we normalize the values of the lines added and the lines deleted of a file by the total lines added and lines deleted.
% Table~\ref{Table:ProcessOwnershipMetrics} provides a summary of the studied process and ownership metrics.


% \todo{Organization metrics} describe the relationship between organizational structure and software quality~\cite{Nagappan2008}.

% MAJOR = major author




==> sections/design.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Study Design}\label{sec:design}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we present the objective of our study, research questions, the studied systems, and software metrics.


\subsection{Research Questions}
The goal of this paper is to better understand the differences in the code ownership approximations and identify the appropriate code ownership approximation that should be used for a software quality management plan.
We present the motivation for our research questions as follows.
% for generating software quality improvement plans.
% help practitioners and researchers \kla{perhaps, only researchers, to be safe} 
% Hence, we conduct two analyses to investigate the difference of code ownership approximations and to analyze the association between the code ownership approximations and software quality.

% \subsubsection*{\analysisI}

\indent \textbf{(RQ1) \rqone}\\
Code ownership approximation can be used to identify owners (or \cnter{s}) for a given source code file. However, approximating code ownership based on a different granularity of contributions may lead to a different set of \cnter{s}.
    Hence, we set out to examine the consistency in terms of the set of \cnter{s} identified by the two approaches.
    % different code ownership approximations capture different aspects of developers' contributions, which could lead to different sets of owners.
% \kla{need some impact statement}
% Yet, little is known about whether both code ownership approximations could identify the common set of authors.
% Thus, we investigate the following research question:~\emph{(RQ1) \rqone}


\indent \textbf{(RQ2) \rqtwo}\\
As discussed in the Motivating Scenarios 1 and 2, the approximated ownership values may be inconsistent even though the \cnter{s} can be identified by both approaches. 
    Then, the set of experts (e.g., major developers) may be inconsistently identified by the two approaches.
    Hence, we set out to analyze the consistency of the approximated ownership values.
% It is likely that a proportion of developers may be considered as a major developer by both the commit-based and line-based code ownership approximations.
% Yet, little is known about whether such common developers that are considered as a major developer by both the commit-based and line-based code ownership approximations have a consistent code ownership value.
% Thus, we investigate the following research question: \emph{(RQ2) \rqtwo}
    % \item 
    
\indent \textbf{(RQ3) \rqthree}\\
As discussed in Motivating Scenario 3, some \cnter{s} who made significant contributions (i.e., major developers) may not be identified by the code ownership approximation.
    Hence, we set out to investigate how many major developers can be missed by using one approach (or another).
%     Finally, a developer may consider as a major developer by the commit-based code ownership approximation, but may not be considered by the line-based code ownership approximation.
% Thus, the contributors of major developers may not be accounted for by one code ownership approximation (and vice versa).
% Thus, we investigate the following research question: \emph{(RQ3) \rqthree}
% \end{enumerate}




% \subsubsection*{\textbf{Analysis II---Identifying the most appropriate code ownership approximations for generating software quality improvement plans.}}


% \subsubsection*{\analysisII}

\indent \textbf{(RQ4) \rqfour}\\
Prior work used defect models to understand the association between code ownership approximations and software quality~\cite{Bird2011a,thongtanunam2016revisiting}.
Such an understanding of defect-proneness is essential
to chart quality management plans, e.g., developing
code ownership policies if code ownership is highly associated with software quality. 
However, it is still unclear about the code ownership approximated by which approach has the strongest association with software quality.

% B. Caglayan, B. Turhan, A. Bener, M. Habayeb, A. Miransky, and E. Cialini. Merits of Organizational Metrics in Defect Prediction: An Industrial Replication.
% In Proceedings of the 37th International Conference on
% Software Engineering, pages 89–98, 2015.
% M. Greiler, K. Herzig, and J. Czerwonka. Code Ownership and Software Quality: A Replication Study. In
% Proceedings of the 12th International Working Conference on Mining Software Repositories, pages 2–12,
% 2015
% N. Nagappan, B. Murphy, and V. R. Basili. The Influence of Organizational Structure on Software Quality:
% An Empirical Case Study. In Proceedings of th 30th International Conference on Software Engineering, pages
% 521–530, 2008.


%  relationship between traditional code ownership heuristics and software quality [7, 9, 14, 35].
% Yet, since traditional code
% ownership heuristics do not include code review activity, little is known about the role that reviewing
% plays in ownership and its impact on defect-proneness.
% Hence, we revisit the relationship between code ownership and software quality using review-specific and
% review-aware heuristics.


% \noindent \textbf{(RQ5) \rqfive}\\
% \indent \underline{Motivation:} 
% Recent work~\cite{jiarpakdee2020xai4se} raised a concern that the factors that are highly associated with software quality in a past release ($i-1$) are not always highly associated with software quality in a current release ($i$).
% As such, it is possible that code ownership policies developed based on the data of a previous release may not be effective for a current release.
% Hence, we set out to examine whether the association of code ownership with software quality discovered in a past release applies to a current release or not.

% \noindent \textbf{(RQ6) \rqsix}\\
% \indent \underline{Motivation:} 
% Finally, the most effective software quality improvement plan could be developed based on the most important risk factors in the current release (e.g., a policy to have a commit-based code ownership more than 5\% for a file).
% Yet, little is known about whether the risk of having defects will be reduced if such code ownership is controlled in the quality improvement plans.
% Thus, we investigate the following research question: 


% \pick{Will continue editing RQ6. I think one question we should address is "Should the two approaches combined?". And I think we can combine RQ5 and RQ6.}

% However, prior studies use different code ownership approximations. 
% Thus, we investigate the following research question: \emph{(RQ4) \rqfour}

% For example, Bird~\ea~\cite{Bird2011a,bird2010analysis} used a regression model to investigate the relationship between the commit-based code ownership and software quality, while Rahman and Devanbu~\cite{rahman2013and} investigated the relationship between the line-based code ownership and software quality.

% While prior work \cite{Bird2011a,bird2010analysis,rahman2013and} suggested that software quality improvement plans can be developed based on the insights that


% Recently, Jiarpakdee~\ea~\cite{jiarpakdee2020xai4se} raised concerns that the most important factors of defect models trained on a past release ($i-1$) are not always important in a current release ($i$).
% As such, it is likely that code ownership that is important in the past release may not always be important in the current release.
% A better understanding of the most important code ownership approximations in the current release is need to chart the most effective software quality improvement plans.
% In other words, the allocation of the software quality assurance resources may be sub-optimal if the most important risk factors are not applied.
% Thus, we investigate the following research question: \emph{(RQ5) \rqfive}


% Finally, the most effective software quality improvement plan could be developed based on the most important risk factors in the current release (e.g., a policy to have a commit-based code ownership more than 5\% for a file).
% Yet, little is known about whether the risk of having defects will be reduced if such code ownership is controlled in the quality improvement plans.
% Thus, we investigate the following research question: \emph{(RQ6) \rqsix}


% Yet, it has not been investigated in prior work~\cite{Bird2011a,bird2010analysis,rahman2013and}.
% Yet, little is known about whether code ownership is also important in a current release.
% Thus, it is likely that different files in the current releases may have different most important risk factors.
% For example, code ownership might be the most important factor for a file, while churn is the most important factor for the other files.
% Thus, a fine-grained understanding of the most important risk factor for each file is very crucial to develop a specific quality improvement plan, instead of relying on the most important factor that is derived from the model level.
% However, such fine-grained understanding is still challenging.
% To the best of our knowledge, there no study exists that investigate the extent to which code ownership policy that is derived from historical data hold true for files in the current releases.
% The understandings of the most important factors that impact software quality is important to chart software quality improvement plans.
% Such understandings are often derived from analytical models trained on historical data.

% quality improvement plans could be used to 
% \kla{empharize that bird and devanbu never evaluate with the future}

% Despite a model-agnostic technique can be used to generate explanations, developers often do not know what should they do to mitigate the risk of having defects.
% Thus, we develop a framework to generate software quality improvement plans using a LIME's model-agnostic technique.
% Importantly, we want to investigate when controlling for code ownership in the quality improvement plans, will the risk of having defects be reduced.


% have different characteristics.
% However, when developing software 
% In other words, such knowledge that is discovered in the past is only
% Yet, little is known if such knowledge also hold true for each file in the next release.
% Specifically, 

% Despite both
% The knowledge the impact of code ownership on software quality from the knowledge
% \kla{when knowledge is derived from historical data, does such knowledge still hold true for the next release}
% \kla{empharize that bird and devanbu never evaluate with the future}

% investigate the relationship between the commit-based code ownership and software quality

% The signals that code ownership has an impact on software quality indicates that code ownership could be a good predictor to identify which files have the highest risk of having software defects.
% Thus, SQA resources should be prioritized to that files.
% However, practitioners often do not understand why such files are predicted as most defective.
% Recently, Jiarpakdee~\ea~\cite{jiarpakdee2020xai4se} raised concerns that a lack of explainability of defect models could lead to a lack of adoption in practices.
% Despite we could explain defect models using various techniques like ANOVA for logistic regression and the variable importance analysis for random forest, such explanations are derived at the model level from historical data and do not specific to each file under prediction in the current releases.
% Therefore, Jiarpakdee~\ea~\cite{jiarpakdee2020xai4se} suggested that a model-agnostic technique is needed to generate explanations of the predictions of defect models.




% To better understand the review dynamics of modern
% transparent code review processes and the impact of
% such dynamics on software quality, we perform an empirical study using a two-fold analysis. Figure 1 provides
% an overview of our case study design, which we briefly
% describe blow

% The hypothesis of Commit-based Approximation.

% \cite{foucault2014code} no impact for FLOSS


% situate the two analyses

% to investigate the differences

% and which one is the best?


% The goal of this paper is to investigate the difference and the importance of code ownership approximations for generating quality improvement plans.
% To achieve this goal, we conduct an empirical study using a statistical approach to address the following six research questions along two perspectives.

% % \subsubsection*{Part 1 - Analyzing the Difference of Code Ownership Approximations.}

% data / source code / history
% - contributors - who contribute to a file, regardless the amount of contributions
% - ownership value (used to identify who own this code, who should be responsible for, acknowledgement in OSS) = amount of contributions  / different approximations may produce different value, ()
% - 



% First, we analyze the importance of code ownership approximations based on the importance scores of the Random Forest classifiers.
% Since such importance scores are derived based on historical data, they may not be applicable to the current predictions and applicable to future releases.

% Thus, we analyze the importance of code ownership approximations using a cross-release scenario with three consecutive releases.
% A release $i$, a release is used to generate the importance scores of defect analytical models, a release $j$ is used to test the explanations of the predictions of defect analytical models, and a release $k$ is used to validate if such explanations are applicable to generate quality improvements plans to minimize the risks of having defects.

% \subsection{Motivation}


% \subsection{Motivation and Research Questions}

% To better understand the review dynamics of modern
% transparent code review processes and the impact of
% such dynamics on software quality, we perform an empirical study using a two-fold analysis. Figure 1 provides
% an overview of our case study design, which we briefly
% describe blow.


% we aim to investigate the differences of code ownership approximations and their impact on software quality.
% Specifically, we investigate if commit-based and line-based code ownership approximations produce the same set of authors, identify the same set of major developers, and produce the same ownership values.
% Then, we investigate which code ownership approximations have the strongest impact on software quality, do such finding hold true on unseen data, would the risk of having defects will be mitigated when controllilng for code ownership.




\subsection{Studied Systems}
In this work, we use a corpus of publicly-available defect datasets provided by Yatish~\ea~\cite{yatish2019mining} where the ground truths were labelled based on the affected releases. 
% We did not use the other publicly-available defect datasets which use the approximation of a post-release window (e.g., 6 months) to identify post-release defects 
We opt to use these datasets because prior work~\cite{yatish2019mining}  showed that when using the approximation of a post-release window (e.g., 6 months) to identify post-release defects, (1) some issue reports addressed within the post-release window do not affect a studied release (false positive), while (2) some issue reports that affect the studied release can be addressed later than the post-release window (false negative). 

The datasets consist of 32 releases that span across 9 open-source software systems. 
Each dataset has 59 software metrics along two
dimensions, i.e., 54 product metrics and 5 process metrics. 
Table~\ref{studied_datasets} presents a summary of the studied systems.




\input{sections/data_preparation}







% \subsection{Motivation and Research Questions}
% The results of Part I show that commit-based and line-based code ownership approximations (1) have different assumptions, (2) identify different set of authors, (3) produce different ownership values, and (4) major authors could be missed by either commit-based or line-based code ownership approximations.
% Despite prior studies found that code ownership has an impact on software quality, they only focus on one individual code ownership approximation.
% Yet, little is known about which code ownership approximation has the strogest impact on software quality.
% Thus, we formulate the following research question: 
% % (RQ4) Which code ownership approximations have the strongest impact on software quality?




% RQ4: Which code ownership approximations have the strongest impact on software quality?


% Analyzing the association betwen code ownership approximations and defect-proneness.




% rq5 - different files have different characteristics

% rq6 - actionable QA plans


% benefits of code ownership - , different approximations may impact the identification of contributors, 

% A better understanding of the difference of approximations will help practitioners and future research to select an appropriate approximation based on the goal.

% Knowing the strongest impact on software quality will suggest managers which aspect to be more focused when developing quality improvement plans.






% \emph{(RQ4) \rqfour} 

% % The analysis 


% % what is best approximation for generating quality improvement plans

% % - files, not tooo minor people, 
% % - minor people review, need major people
% % - rahman suggested? file level

% % but different approximations could draw quality improvement plans
% % - but what is the most important factor of software quality?

% % thus, we build a defect model

% Since the importance scores of code ownership approximations are derived from defect  models that are built from the historical data, such importance scores may not be applied to all predictions.
% Recently, Jiarpakdee~\ea~\cite{jiarpakdee2020xai4se} found that different defective files have different characteristics and different explanations on why a file is predicted as defective. 
% - explainability - 
% Yet, little is known if 
% % specific groups of files / commit is better than file.
% % are they applicable to all files

% \noindent \emph{(RQ5) \rqfive}
% % (RQ5) Should code ownership approximations be used to explain why a file is predicted as defective?

% [code ownership policy / code ownership management]
% Software Quality Assurance (SQA) planning is the process of developing proactive SQA plans to define the quality requirements of software products and processes 
% \cite{galin2018software}.
% Such proactive SQA plans will be used as guidance to prevent software defects that may slip through to future releases.
% The first SQA planning activity is to define the scope of product and process measurements, operationalize metrics, and identify risk thresholds~\cite{maxim2016introduction}.

% Unfortunately, current analytical modelling approaches do not provide a risk threshold i.e., what is the optimal threshold of code review expertise to maintain the quality of a file. Thus they cannot generate the following types of guidance:

% A lack of such types of actionable guidance to support software quality improvement planning leads to ineffective and inefficient SQA practices~\cite{sowunmi2016empirical}. This poses a critical challenge to release-based SQA practices in many software projects.

% we propose a framework to generate Code-Ownership-based SQA Policy.





% % To  answer  RQ6,  we  investigate  the  proportionof  QA  improvement  plans  generated  by  LIME  that  areapplicable  to  guide  contributors  to  minimize  the  risks  ofhaving  defects  for  the  subsequent  release  (i.e.,  a  releasek).  Given  a  QA  improvement  plan  of  a  defective  file  of{LOC<=100} ⇒CLEAN, 

% \noindent \emph{(RQ6) \rqsix} We investigate ...
% % (RQ6) How applicable is the quality improvement plan based on code ownership approximation?





% The goal of this analysis is to investigate \kla{??}.

% First, we analyze the importance of code ownership approximations based on the importance scores of the Random Forest classifiers.
% Since such importance scores are derived based on historical data, they may not be applicable to the current predictions and applicable to future releases.

% Thus, we analyze the importance of code ownership approximations using a cross-release scenario with three consecutive releases.
% A release $i$, a release is used to generate the importance scores of defect analytical models, a release $j$ is used to test the explanations of the predictions of defect analytical models, and a release $k$ is used to validate if such explanations are applicable to generate quality improvements plans to minimize the risks of having defects.

==> sections/table_studied_metrics.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}
\caption{A summary of the product metrics.}
\label{Table:CodeMetrics}
 \centering
 % \setlength\arrayrulewidth{1pt}
 \begin{tabular}{p{0.065\linewidth}p{0.835\linewidth}p{0.0325\linewidth}}
 \hline
 \textbf{Granularity} & \textbf{Metrics} & \textbf{Count}\\
 \hline
 File & AvgCyclomatic, AvgCyclomaticModified, AvgCyclomaticStrict, AvgEssential, AvgLine, AvgLineBlank, AvgLineCode, AvgLineComment, CountDeclClass, CountDeclClassMethod, CountDeclClassVariable, CountDeclFunction, CountDeclInstanceMethod, CountDeclInstanceVariable, CountDeclMethod, CountDeclMethodDefault, CountDeclMethodPrivate, CountDeclMethodProtected, CountDeclMethodPublic, CountLine, CountLineBlank, CountLineCode, CountLineCodeDecl, CountLineCodeExe, CountLineComment, CountSemicolon, CountStmt, CountStmtDecl, CountStmtExe, MaxCyclomatic, MaxCyclomaticModified, MaxCyclomaticStrict, RatioCommentToCode, SumCyclomatic, SumCyclomaticModified, SumCyclomaticStrict, SumEssential & 37\\
 \cline{1-3}
 Class & CountClassBase, CountClassCoupled, CountClassDerived, MaxInheritanceTree, PercentLackOfCohesion & 5\\
 \cline{1-3}
 Method & CountInput\_\{Min, Mean, Max\}, CountOutput\_\{Min, Mean, Max\}, CountPath\_\{Min, Mean, Max\}, MaxNesting\_\{Min, Mean, Max\} & 12\\
 \hline
 \end{tabular}
\hspace{\fill}
\end{table*}


\renewcommand{\arraystretch}{1.2}
\begin{table}
\caption{A summary of the process metrics.}
\label{Table:ProcessMetrics}
\resizebox{.99\columnwidth}{!}{ 
\centering
% \setlength\arrayrulewidth{1pt}
\begin{tabular}{p{0.23\linewidth}p{0.8\linewidth}}
\hline
\textbf{Metrics} & \textbf{Description}\\
\hline
% \multicolumn{2}{l}{\emph{Ownership Metrics}}    \\
% \hline
% OWN\_COMMIT & The proportion of code changes (i.e., Git commits) made by the developer who has the highest contribution of code changes on the module\\ 
% OWN\_LINE & The proportion of lines of code written by the developer who has the highest contribution of lines of code on the module \\
% MAJOR\_COMMIT & The number of unique developers who have contributed more than 5\% of the total code changes (i.e., Git commits) on the module \\
% MAJOR\_LINE & The number of unique developers who have contributed more than 5\% of the total lines of code on the module\\
% MINOR\_COMMIT & The number of unique developers who have contributed less than 5\% of the total code changes (i.e., Git commits) on the module\\
% MINOR\_LINE & The number of unique developers who have contributed less than 5\% of the total lines of code on the module\\ 
% \hline
% \multicolumn{2}{l}{\emph{Process Metrics}}    \\
% \hline
COMM & The number of Git commits\\
ADDED\_LINES & The normalized number of lines added to the module \\
DEL\_LINES & The normalized number of lines deleted from the module \\
ADEV & The number of active developers\\
DDEV & The number of distinct developers\\
\hline
\end{tabular}}
\end{table}
